A Two-Prong Approach to Energy-Efficient WSNs: Wake-Up Receivers plus Dedicated, Model-Based Sensing

Energy neutral operation of WSNs can be achieved by exploiting the idleness of the workload to bring the average power consumption of each node below the harvesting power available. This paper proposes a combination of state-of-the-art low-power design techniques to minimize the local and global impact of the two main activities of each node: sampling and communication. Dynamic power management is adopted to exploit low-power modes during idle periods, while asynchronous wake-up and prediction-based data collection are used to opportunistically activate hardware components and network nodes only when they are strictly required. Furthermore, the concept of "model-based sensing" is introduced to push prediction-based data collection techniques as close as possible to the sensing elements. The results achieved on representative real-world WSN case studies show that the combined benefits of the design techniques adopted is more than linear, providing an overall power reduction of more than 3 orders of magnitude.

==> relwork-b4-alm.tex <==
\section{Background and Related Work}\label{sec:relwork}


This section offers background on the techniques used throughout this paper to
effectively exploit DPM: prediction-based data collection, wake-up
receivers and ultra low-power sensor nodes.

%First, \pbdc is a software solution that lowers the data rate of the application without sacrificing data accuracy. Second, several motes provide advanced DPM features that enable the WSN programmers to turn off various hardware components between idle periods. Third, a wake-up receiver is a hardware solution that consumes less energy than a standard duty cycling MAC protocol by avoiding the consumption due to idle listening that would occur between the infrequent transmissions generated by the first approach.


\subsection{\Pbdc} 
\label{subsec:pbdc}

As a first step toward reducing consumption, we turn to techniques that reduce
the data that must be transmitted. Many such techniques exist such as data
compression, in-network data processing and data aggregation~\cite{anastasi2009energy}, but we focus on \pbdc due to its
simplicity and demonstrated effectiveness on the scenarios we target.

In \pbdc, the original application sampling frequency is maintained, but the
total amount of data transmitted is reduced~\cite{anastasi2009energy} by
generating a model for the sensed data. This model is used at the sink to
approximate the sampled data points.  With each new sample, the node verifies
that it falls within allowable error tolerances.  If so, no action is taken,
but if not, a new model is generated and transmitted to the sink.  If the
model closely approximates the data trend, the network communication is
significantly reduced, up to 99\% in some
cases~\cite{raza12:what,edgemining,pwsn}. Various types of models have been
studied.  Probabilistic
models~\cite{DBLP:conf/vldb/DeshpandeGMHH04,DBLP:conf/icde/ChuDHH06}
approximate data with a user-specified confidence, but special data
characteristics must be encoded by domain experts.  Alternate techniques
employ linear regression~\cite{DBLP:conf/ewsn/TuloneM06}, autoregressive
models~\cite{DBLP:conf/mswim/TuloneM06} and Kalman
filters~\cite{Jain:2004:ASR:1007568.1007573}, but with sizeable memory and
computational requirements, making them difficult to implement on
resource-limited motes. A simpler, linear approach~\cite{raza12:what},
detailed in Section~\ref{sec:dbp}, was recently proposed by some of the
authors of this paper, and is adopted for the case study here.

%Additional classes of data reduction techniques include data compression, in-network data processing and data aggregation~\cite{anastasi2009energy}. Although they can be used in conjunction with \pbdc, the additional complexity outweighs the benefit for many WSN applications. Specifically, in the case studies explored in Section~\ref{sec:results}, \pbdc alone achieves sufficient savings, therefore we did not consider the addition of these other techniques.


\subsection{Wake-up Receiver} 
Wake-up receivers are a viable solution to enable low-power, asynchronous
communication, essentially by triggering the activation of the primary
radio~\cite{lin04}. Several wake-up solutions have recently been
developed~\cite{hambeck11,huang11,marinkovic11,petrioli14,magno14,magnotii14},
each optimizing different parameters such as working power, sensitivity,
distance range, latency, and operating frequency. These solutions use the
radio channel to convey triggering signals, but alternative proposals use
out-of-band signals such as ultrasound. Notably, this paper evaluates an
ultrasonic wake-up module for the VirtualSense platform recently developed by
some of the authors of this paper~\cite{lattanziUS13}, as it outperforms
state-of-the-art radio wake-up receivers with a sub-$\mu$A quiescent current
consumption.

Recent researches have shown the potential for asynchronous wake-up schemes
in some application scenarios~\cite{jelicic12,sies14}. Specifically,
studies~\cite{tn,petrioli} have shown that, in comparison to duty
cycling protocols, wake-up receivers offer longer system lifetimes, lower
latency, and better reliability in multiple application domains. These studies
note that wake-up receivers are particularly effective for applications with
ultra-low traffic, as they avoid the idle listening incurred at routing nodes
to periodically check for incoming packets.  This paper builds on this
observation, specifically showing how traditional applications with moderate
data rates can be converted into ultra-low traffic applications with \pbdc,
thus enhancing the effectiveness of wake-up receivers and DPM.

\subsection{Ultra-low Power Platforms}
Careful design of embedded wireless hardware platforms is key to energy
efficient WSNs. Over the last 15 years, many efforts have been devoted to
devise novel ultra-low power MCUs and radio transceivers.  \amy{cut (the
  history is not necessary): First generation WSN platforms included
  Rene~\cite{hill00}, Mica~\cite{hill02} and
  Telos~\cite{polastre05}. Afterwards, the design of embedded architectures
  for sensor nodes has mainly relied on 16-bit MCUs and IEEE 802.15.4
  compliant transceivers. } Recent trends show a shift towards 32-bit
platforms that meet strict WSN energy requirements~\cite{andersen14}. All of
these platforms come with the ability to opportunistically turn off hardware
components in periods of idleness. The next section details VirtualSense, the
platform designed by some of the authors of this paper, focusing on the
various elements it offers for dynamic power management.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

